Provable Burer-Monteiro factorization for a class of norm-constrained matrix problems

We study the projected gradient descent method on low-rank matrix problems with a strongly convex objective. We use the Burer-Monteiro factorization approach to implicitly enforce low-rankness; such factorization introduces non-convexity in the objective. We focus on constraint sets that include both positive semi-definite (PSD) constraints and specific matrix norm-constraints. Such criteria appear in quantum state tomography and phase retrieval applications. We show that non-convex projected gradient descent favors local linear convergence in the factored space. We build our theory on a novel descent lemma, that non-trivially extends recent results on the unconstrained problem. The resulting algorithm is Projected Factored Gradient Descent, abbreviated as ProjFGD, and shows superior performance compared to state of the art on quantum state tomography and sparse phase retrieval applications.

==> FGD.tex <==
\section{The factored gradient descent (\algo) algorithm}\label{sec:FGD}
Let us first succinctly describe \algo algorithm, upon which our proposed scheme is based. 
We remind that \algo solves \eqref{intro:eq_00} for $\C \equiv \R^{n \times r}$.
The pseudocode for \algo is provided in Algorithm \ref{algo:FGD}.
The initial point satisfies $\X_0 := \sfrac{1}{\widehat{L}} \cdot \Pi_{+}\left(-\nabla f(0) \right)$, where $\Pi_{+}(\cdot)$ denotes the projection onto the set of PSD matrices and $\widehat{L}$ represents an approximation of $L$; see \cite{bhojanapalli2015dropping}.
The main iteration of \algo applies the simple rule 
%\begin{align*}
$\U_{t+1} = \U_t - \eta \gradf(\U_t\U_t^\top)  \cdot \U_t$,
%\end{align*} 
with step size:
\begin{align}\label{eq:step_size}
\eta \leq \tfrac{C}{L\norm{\X_0}_2 + \norm{\gradf(X_0) }_2},
\end{align}
which lead to the following guarantees, when $f$ is $L$-smooth and strongly convex:

\begin{theorem}\label{thm:FGD_guarantees}
Let $\U_t$ be the current estimate and $\X_t = \U_t\U_t^\top$. 
Assume the optimum of $f$ $\X^\star := \U^\star \U^{\star \top}$ is rank-$r$, and $ \dist(\U_t, \Uo) \leq \rho' \sigma_{r}(\Uo)$, for $\rho' := c \cdot \tfrac{\mu}{L} \cdot \tfrac{\sigma_r(\X^\star)}{\sigma_1(\X^\star)}$ and $c \leq \tfrac{1}{100}$ constant. 
Let the step size follow \eqref{eq:step_size}, with $C = \tfrac{1}{16}$. 
Then, the recursion $\U_{t+1}= U_t -\eta \nabla f(\U_t \U_t^\top) \cdot U_t$ satisfies
\begin{equation}
\dist(\U_{t+1}, \Uo)^2 \leq \alpha \cdot \dist(\U_t, \Uo)^2, \label{conv:eq_00}
\end{equation}
where $\alpha = 1 - \frac{\mu \sigma_{r}(\Xo)}{64 (L\|\Xo\|_2 + \|\gradf(\Xo)\|_2)} < 1$, i.e., the algorithm shows linear convergence. 
Furthermore, $\U_{t+1}$ satisfies $ \dist(\U_{t+1}, \Uo) \leq \rho' \sigma_{r}(\Uo). $
\end{theorem}

\begin{wrapfigure}{r}{0.5\textwidth} 
   \vspace{-1.5em}
\begin{minipage}{0.52\textwidth}
	\begin{algorithm}[H]
		\caption{Factored gradient descent (\algo)} \label{algo:FGD}
		\begin{algorithmic}[1]		
			\INPUT Function $f$, target rank $r$, \# iterations $T$. 
			\STATE Compute $\X_0 := \sfrac{1}{\widehat{L}} \cdot \Pi_{+}\left(-\nabla f(0) \right)$.
			\STATE Set $\U_0 \in \R^{n \times r}$ such that $\X_0 = \U_0\U_0^\top$.
			\STATE Set step size $\eta$ as in \eqref{eq:step_size}.
			\FOR {$t=0$ to $T-1$}
				\STATE $\U_{t+1} = \U_t - \eta \gradf(\U_t\U_t^\top)  \cdot \U_t$.
			\ENDFOR
			\OUTPUT $\X = \U_T\U_T^\top$. 	
		\end{algorithmic}
	\end{algorithm}
\end{minipage}
	 \vspace{-1em}
\end{wrapfigure}
Key ingredients to achieve the above guarantee are the initialization --so that $\dist(\U_0, \Uo)$ is sufficiently small-- and the step size selection. 
For the initialization, as the authors of \cite{bhojanapalli2015dropping} state, one could use either the expression in Algorithm \ref{algo:FGD} or more specialized spectral methods; see \cite{chen2015fast, zheng2015convergent}. 
Alternatively, one could even run algorithms applied on the original variable space \eqref{intro:eq_01} for only a few iterations --and thus might include some full or truncated SVDs; see \cite{tu2015low} for the case of matrix completion/sensing.

%\paragraph{Step size $\eta$.} Even though $f$ is a proper convex function over $X\succeq 0$, the fact that we operate with the non-convex $\U\U^\top$ parametrization means that we need to be careful about the step size $\eta$; \textit{e.g.}, our \emph{constant} $\eta$ selection should be such that, when we are close to $\Xo$, we do not ``overshoot'' the optimum $\Xo$. In \cite{bhojanapalli2015dropping}, the step size proposed, that can guarantee convergence under some assumptions, is of the form\footnote{Specifically, \cite{bhojanapalli2015dropping} suggest $C = 16$. The exact value of $C$ depends on how good the initialization is and by the nature of the problem. It is important, though, that $\eta$ scales inversely proportional to $L\norm{\X^\star}_2 + \norm{\gradf(X^\star) }_2$.}
 %Recall that, if we were just doing standard gradient descent on $f$, we would choose a step size of $\sfrac{1}{M}$, where $M$ is a uniform upper bound on  the largest eigenvalue of the Hessian $\nabla^2 f(\cdot)$.


==> proj_fgd.tex <==

%%%%%%%%%%%%%%%%%%%%
\section{Appendix D - Old proof}
We consider the problem $min~ f(X), X \succeq 0 \text{~and~} X \in C_X$ and re-parametrize to $min~ f(UU^\top),~ U \in C_U$. We assume $C_X$ is a convex set over $X$ and there exists a corresponding $C_U$ a convex set over the factor space $U$. Further we assume if $U \in C_U$ then, $UU^\top \in C_X$. Now we consider optimizing this problem using projected gradient descent over the factor space $U$. 

Hence the updates are, $\Uhp = U -\eta \gradf(X)U$ and $\Up=D\cdot \Uhp$. D is a diagonal matrix. %Define $\gU = \frac{1}{\eta}(U -\Up)$ and $\gX = \frac{1}{\eta}\left(Q_U Q_U^\top -\PU(U-\eta\gradf(X)U)U^\dagger \right)$. Then, $\gU =\gX*U$.

\begin{theorem}
$$\dist(\Up, \Uor)^2 \leq (1 -\frac{3m \sigma_r(\Xo)\eta}{10}) \| \Delta\|_F^2+ \frac{17M \eta}{32} \norm{\Xo -\Xor}_F^2.$$
\end{theorem}

\begin{proof}
For the proof we will work with step size $\eta =\frac{1}{16(M||X||_2 +||\gradf(X)||_2)}$. This is equivalent upto constants to the original step size in the algorithm. {\color{red}(see lemma ref)}

\begin{align*}
    \dist(\Up,\Uor)^2 &\leq ||\Up -\Uor||_F^2 \\
    &=||\Up-U+U-\Uor||_F^2\\
    &=||\Up -U||_F^2 +||U-\Uor||_F^2-2\ip{U-\Up}{U-\Uor}.
    %&=||U-\Uor||_F^2-||\Up -U||_F^2 -2\ip{U-\Up}{\Up-\Uor}\\
   % &\leq ||U-\Uor||_F^2-||\Up -U||_F^2 -2\ip{U-\Uhp}{\Up-\Uor}.
\end{align*}
%For the last step, recall $\Up$ is projection of $\Uhp$. Hence, $\ip{\Uhp-\Up}{\Up -\Uor} \geq 0$. This implies, $\ip{U-\Up}{\Up -\Uor} \geq \ip{U - \Uhp}{\Up -\Uor}$.

Now we will bound the inner product in the above.
\begin{align*}
    \ip{U-\Up}{\U-\Uor}&=\ip{U-D(U-\eta\gradf(X)U)}{\U-\Uor}\\
    &=\ip{U-DU}{\U -\Uor}+\eta\ip{D\gradf(X)U}{\U-\Uor}.
\end{align*}
Now using Lemma~\ref{lem:gradU,U-U_r_ bound} we get,
\begin{align*}
      \dist(\Up,\Uor)^2 &\leq ||\Up -U||_F^2 +||U-\Uor||_F^2-2\ip{U-DU}{\U -\Uor} \\ &\quad\quad -\frac{2\eta}{d} \left(\frac{17}{16\eta} ||U- \Up||_F^2  +\tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 +\frac{1}{20\eta}(1-\frac{1}{d})||U||_F^2- \tfrac{M}{4}\norm{\Xo -\Xor}_F^2\right) \\
      &\leq ||\Up -U||_F^2 +||U-\Uor||_F^2 + \frac{2}{100}(1-\frac{1}{d}) ||U||_F^2  \\ &\quad \quad -\frac{2*17\eta}{16} \left(\frac{17}{16\eta} ||U- \Up||_F^2 +\frac{1}{20 \eta}(1-\frac{1}{d})||U||_F^2 +\tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2- \tfrac{M}{4}\norm{\Xo -\Xor}_F^2\right) \\
      &\leq (1 -\frac{3m \sigma_r(\Xo)\eta}{10}) \| \Delta\|_F^2+ \frac{17 M \eta}{32} \norm{\Xo -\Xor}_F^2  +\left(\tfrac{2}{100} -\tfrac{17}{160} \right)(1-\tfrac{1}{d}) ||U||_F^2  \\
      &\leq \leq (1 -\frac{3m \sigma_r(\Xo)\eta}{10}) \| \Delta\|_F^2+ \frac{17 M \eta}{32} \norm{\Xo -\Xor}_F^2
\end{align*}
\end{proof}

\subsection{Proof of Lemma~\ref{lem:gradU,U-U_r_ bound}}\label{sec:supp_sc3}
\begin{lemma}[Descent lemma]\label{lem:gradU,U-U_r_ bound}
%Let $\|\Delta\|_F \leq  \rho'\sigma_{r}(\Uo_r)$ and $\|\Xo -\Xo_r\|_F \leq \frac{\rho'}{2\sqrt{\kappa}} \sigma_r(\Xo)$, where $\rho'=\frac{1}{100 \kappa \tau(\Xo_r)}$. Then, 
For $f$ being a $M$-smooth and $(m, r)$-strongly convex function and under assumptions $(A2)$ and $(A4)$, the following inequality holds true:
\begin{align*}
\ip{\gradf(X)U}{\U -\Uorr} \geq  &\frac{17}{16\eta} ||U -\Up||_F^2 + \frac{47 \cdot \eta}{160}  \|\gradf(X) U\|_F^2 + \tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 \\&\quad \quad +\frac{1}{20 \eta}(1-\frac{1}{d})||U||_F^2 -\tfrac{M}{4}\norm{\Xo -\Xor}_F^2 .
\end{align*}
\end{lemma}

\begin{proof}
Recall $\Uhp =U -\eta\gradf(X)U$. First we rewrite the inner product as shown below.
\begin{align}
\ip{\gradf(X)U}{\U -\Uorr}&= \ip{\gradf(X) }{\X -\Uorr \U^\top} \nonumber \\
&=\frac{1}{2}\ip{\gradf(X) }{\X -\Xo_r}  + \ip{\gradf(X) }{\frac{1}{2}(\X + \Xo_r) -\Uorr \U^\top} \nonumber \\
&=\frac{1}{2}\ip{\gradf(X) }{\X -\Xo_r}  + \frac{1}{2} \ip{\gradf(X) }{\Delta \Delta^\top}, \label{proofsr1:eq_09}
\end{align} which follows by adding and subtracting $\tfrac{1}{2}\Xo_r$. 

Note that by lemma~{\color{red} ref FGD c.1} we know that, $\ip{\gradf(X) }{\Delta \Delta^\top} \leq \frac{1}{40 \kappa \tau(\Xo_r)} ||\gradf(X)U||_F ||\Delta||_F$. By Lemmas \ref{lem:DD_bound} and \ref{lem:gradX,X-X_r_ bound}, we have:

\begin{align*}
& \ip{\gradf(X) \U}{\U -\Uorr}\\ &\geq \frac{17}{16\eta} ||U -\Up||_F^2 + \tfrac{3\cdot\eta}{5 d^2} \|\gradf(X) U\|_F^2 + \tfrac{m}{4}\norm{\X -\Xor}_F^2 +\frac{1}{20 \eta}(1-\frac{1}{d})||U||_F^2 - \tfrac{M}{4}\norm{\Xo -\Xor}_F^2 \\
&\quad \quad \quad \quad \quad \quad \quad \quad- \tfrac{1}{2}\tfrac{1}{80 \kappa \tau(\Xo_r)}\left(   \eta||\gradf(X)U||_F^2 + \frac{1}{\eta}||\Delta||_F^2 \right) \nonumber \\
&= \frac{17}{16\eta} ||U -\Up||_F^2 + \left(\tfrac{3}{5*2}- \tfrac{1}{160}\right) \cdot \eta  \|\gradf(X) U\|_F^2 + \tfrac{m}{4}\left(\norm{\X -\Xor}_F^2 -  \tfrac{1\sigma_{r}(\Xo) }{40} \cdot \| \Delta\|_F^2 \right) \nonumber \\ 
&\quad \quad \quad \quad \quad \quad \quad \quad +\frac{1}{20 \eta}(1-\frac{1}{d})||U||_F^2 - \tfrac{M}{4}\norm{\Xo -\Xor}_F^2 \nonumber \\
&\stackrel{(i)}{\geq} \frac{17}{16\eta} ||U -\Up||_F^2 + \frac{47 \cdot \eta}{160}  \|\gradf(X) U\|_F^2 + \tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 +\frac{1}{20\eta}(1-\frac{1}{d})||U||_F^2 -\tfrac{M}{4}\norm{\Xo -\Xor}_F^2 \nonumber 
%&\stackrel{(ii)}{\geq }\frac{1}{ \eta} ||U- \Up||_F^2 + \tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 - \tfrac{M}{4}\norm{\Xo -\Xor}_F^2
\end{align*}
\end{proof}


\subsection{Proof of Lemma \ref{lem:gradX,X-X_r_ bound_sc}}\label{sec:supp_sc1}


\begin{lemma}\label{lem:gradX,X-X_r_ bound_sc}
Let $f$ be a $M$-smooth and $(m, r)$-restricted strongly convex function with optimum point $\Xo$. Let $\X = \U\U^\top$. Then,
\begin{align*}   
\ip{\gradf(\X)}{\X-\Xor}  \geq &\frac{17}{16\eta} ||U -\Up||_F^2 + \tfrac{3\cdot\eta}{5 d^2} \|\gradf(X) U\|_F^2  +\tfrac{m}{2}\norm{\Xor -\X}_F^2 \\&+\frac{1}{20 \eta}(1-\frac{1}{d})||U||_F^2 -\tfrac{M}{2}\|\Xo -\Xor\|_F^2,
\end{align*}
where  
\end{lemma}

\begin{proof}

Now we will show the lower bound $\ip{\gradf(\X)}{\X -\Xo}$. Our proof differs from the standard convex gradient descent proof (see ~\cite{nesterov2004introductory}) as we need to analyze updates without any projections. Also we construct a pseudo iterate $\Uhp$ to obtain a bigger lower bound than the error term in Lemma~\ref{lem:DD_bound_sc}. Here the step size plays a key role in achieving the bound. 

By smoothness of $\f$, we get:
\begin{align}
\f(\X) &\geq \f(\Xp) -\ip{\gradf(\X)}{\Xp -\X} - \tfrac{M}{2} \norm{\Xp -\X}_F^2 \nonumber \\ 
&\stackrel{(i)}{\geq} \f(\Xo) -\ip{\gradf(\X)}{\Xp -\X} - \tfrac{M}{2} \norm{\Xp -\X}_F^2 , \label{eq:gradX,X-X_r_00}
 \end{align}
where $(i)$ follows from optimality of $\Xo$ and since $\Xp$ is a feasible point $(\Xp \succeq 0, \Pi(\Xp) =\Xp)$ for problem~\eqref{intro:eq_00}. 

Finally, since $\text{rank}(\Xo) = r$, by the $(\rscm, r)$-restricted strong convexity of $\f$, we get, 
\begin{align} 
\f(\Xo) \geq \f(\X) +\ip{\gradf(\X)}{\Xo-\X} +\tfrac{m}{2}\norm{\Xo -\X}_F^2 .\label{eq:gradX,X-X_r_02}
\end{align}
Combining equations~\eqref{eq:gradX,X-X_r_00}, and~\eqref{eq:gradX,X-X_r_02}, we obtain: 
\begin{small}
\begin{align} 
\ip{\gradf(\X)}{\X-\Xo} \geq  \ip{\gradf(\X)}{\X -\Xp} -\tfrac{M}{2} \norm{\Xp -\X}_F^2+\tfrac{m}{2}\norm{\Xo -\X}_F^2  \label{eq:gradX,X-X_r_03} 
\end{align}
\end{small}
It is easy to verify that $\Xp =  \frac{1}{d^2}\left(\X - \eta \gradf(\X) \X \Lambda - \eta \Lambda^\top \X \gradf(\X)\right)$, where $\Lambda = I - \tfrac{\eta}{2} Q_U Q_U^\top \gradf(X) \in \R^{n \times n}$. 
%In the proof that follows, we use as step size $\widehat{\eta} = \tfrac{1}{16 (M\|\X\|_2 + \|\gradf(\X)Q_U Q_U^\top\|_2)}$. 
%By Lemma \ref{lem:stepsize}, we can verify that $\widehat{\eta} \geq \eta$ and, thus, any theoretical result using $\widehat{\eta}$ as step size automatically applies for the proposed step size $\eta$. 
Notice that for step size ${\eta}$, we have 
\begin{align*}
\Lambda \succ 0, \quad  \|\Lambda\|_2 \leq  1+ \sfrac{1}{32} \quad \text{and} \quad \sigma_{n}(\Lambda) \geq  1- \sfrac{1}{32}.
\end{align*} 

%Now recall that \begin{align*}\Xp &= X - \weta \gradf(X)X -  \weta X \gradf(X)+  \weta^2 \gradf(X)X \gradf(X) \\
%&= X - \weta \left( \gradf(X)X\Lambda  + \Lambda^\top X \gradf(X) \right), \end{align*} where $\Lambda =I -\frac{\weta}{2} Q_{U} Q_{U}^\top \gradf(X)$. Notice that for step size $\weta$ considered $\Lambda \succ 0$,  $\|\Lambda\|_2 \leq  1+ \frac{1}{32}$ and $\sigma_{n}(\Lambda) \geq  1- \frac{1}{32}$.

Substituting the above in~\eqref{eq:gradX,X-X_r_03}, we obtain:
\begin{align*}
 \ip{\gradf(\X)}{\X-\Xor} &- \tfrac{m}{2}\norm{\Xor -\X}_F^2 + \tfrac{M}{2}\|\Xor -\Xo\|_F^2  + \tfrac{M}{2} \norm{X -\Xp}_F^2 \\
 								 &\stackrel{(i)}{\geq} \ip{\gradf(X)}{(1-\frac{1}{d^2})X} + 
 								 \frac{2}{d^2}\eta \ip{\gradf(\X)}{\gradf(X)X \Lambda} \\
 								 %&= 2\weta \trace( \gradf(X) \gradf(X)X \Lambda) - 2M\weta^2 \norm{  \gradf(X)X\Lambda }_F^2 \\
 								 &\stackrel{(ii)}{\geq} \ip{\gradf(X)U}{(1-\frac{1}{d^2})U} + \frac{2}{d^2} \eta \trace( \gradf(X) \gradf(X)X) \cdot \sigma_{n}(\Lambda) \\
 								 &\geq (1-\frac{1}{d^2})\ip{\gradf(X)}{X} + \tfrac{31\cdot\eta}{16 d^2} \|\gradf(X) U\|_F^2.
 				                %&=(1+\frac{1}{d}) (1-\frac{1}{d}) \ip{\gradf(X)U}{U} + \tfrac{31\cdot\eta}{16 d^2} \|\gradf(X) U\|_F^2.
 \end{align*} 
 $(i)$ follows from symmetry of $\gradf(X)$ and $\X$. $(ii)$ follows from $\trace(\gradf(X)\gradf(X)X\Lambda) =\trace(\gradf(X)\gradf(X)UU^\top) -\frac{\eta}{2}\trace(\gradf(X)\gradf(X)UU^\top \gradf(X)) \geq (1 -\frac{\eta}{2} \|Q_U Q_U^\top\gradf(X)\|_2) \|\gradf(\X) U\|_F^2  \geq  (1- \sfrac{1}{32}) \|\gradf(\X) U\|_F^2$.  %$(iii)$ follows by $\weta \leq \tfrac{1}{16M \|\X\|_2}$. Thus, we achieve the desiderata:
 
 Now we will use the above equation to get a bound on $\ip{\gradf(\X)}{\X-\Xor} - \tfrac{m}{2}\norm{\Xor -\X}_F^2 + \tfrac{M}{2}\|\Xor -\Xo\|_F^2 -\frac{17}{16\eta} ||U -\Up||_F^2$.
 \begin{align*}
     \ip{\gradf(\X)}{\X-\Xor} &- \tfrac{m}{2}\norm{\Xor -\X}_F^2 + \tfrac{M}{2}\|\Xor -\Xo\|_F^2 -\frac{17}{16\eta} ||U -\Up||_F^2\\
     &\geq  (1-\frac{1}{d^2})\ip{\gradf(X)}{X} + \tfrac{31\cdot\eta}{16 d^2} \|\gradf(X) U\|_F^2 -(1+ \frac{1}{32} )\frac{17}{16\eta} ||U -\Up||_F^2\\
     &\geq  (1-\frac{1}{d^2})\ip{\gradf(X)}{X} + \tfrac{31\cdot\eta}{16 d^2} \|\gradf(X) U\|_F^2 \\
     &\quad -\frac{33}{32}\frac{17}{16 \eta}\left[(1-\frac{1}{d})^2||U||_F^2 + \frac{\eta^2}{d^2}||\gradf(X)U||_F^2 + 2\eta \frac{1}{d} (1-\frac{1}{d}) \ip{\gradf(X)}{X} \right]\\
     &\geq (1-\frac{1}{d})(1+\frac{1}{34d})\ip{\gradf(X)}{X} + \tfrac{0.96\cdot\eta}{ d^2} \|\gradf(X) U\|_F^2 -\frac{33*17}{32*16 \eta}(1-\frac{1}{d})^2||U||_F^2\\
     &\stackrel{(i)}{\geq} (1+\frac{1}{34d}) \frac{0.85}{\eta}(1-\frac{1}{d})^2||U||_F^2 + \tfrac{0.96\cdot\eta}{ d^2} \|\gradf(X) U\|_F^2 -\frac{33*17}{32*16 \eta}(1-\frac{1}{d})^2||U||_F^2\\
     &\stackrel{(ii)}{\geq} \tfrac{0.96\cdot\eta}{ d^2} \|\gradf(X) U\|_F^2 - \frac{0.22}{\eta}(1-\frac{1}{d})^2||U||_F^2\\
     &\geq \frac{3\cdot\eta}{5 d^2} \|\gradf(X) U\|_F^2 +\frac{1}{20 \eta}(1-\frac{1}{d})||U||_F^2.
 \end{align*}
 $(i)$ follows from applying Lemma~\ref{lem:supp2}. $(ii)$ follows from $d \leq \frac{17}{16}$. Last inequality follows from Lemma~\ref{lem:proj1} and  $(1-\frac{1}{d^2}) \leq (1-\frac{1}{d})$.

 
\end{proof}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:proj}
$$||(1-\frac{1}{d})U||_F \leq (1+\frac{1}{d})\eta ||\gradf(X) U||_F.$$
\end{lemma}
\begin{proof}
Recall that $\Up=\frac{1}{d}(U -\eta \gradf(X)U)$ is a projection of $\Uhp =U -\eta\gradf(X)U$. Hence $$\|U-\Up||_F \leq ||U - \Uhp||_F.$$ This implies,
\begin{align*}
    \weta ||\gradf(X)U||_F &\geq ||U -\Up||_F \\
    &\geq ||(1-\frac{1}{d})U||_F - \frac{1}{d}\eta ||\gradf(X)U||_F.
\end{align*}
Hence $||(1-\frac{1}{d})U||_F \leq (1+\frac{1}{d})\eta ||\gradf(X)U||_F.$
\end{proof}


\begin{lemma}\label{lem:proj1}
$$||(1-\frac{1}{d})U||_F \leq \frac{1.15}{d} \eta ||\gradf(X) U||_F,$$ %when $||(1-\frac{1}{d})U||_F \geq \frac{\kappa \tau(\Xo_r)}{50} \dist(U, \Uo)$.
\end{lemma}
\begin{proof}
From optimality of $\Uo$ we know that $\Uo = \frac{1}{d^*}(\Uo-\eta \gradf(\Xo)\Uo).$ Hence $||(1-\frac{1}{d^*})\Uo||_F = \|\frac{1}{d^*} \eta \gradf(\Xo)\Uo\|_F.$ Notice that $d^* \geq 1 \geq \frac{16}{17}d$, since $d \leq \frac{17}{16}$. Also $||\U||_F \leq \frac{101}{100}||\Uo||_F$ from lemma {\color{red} ref}. Hence we get,
$$||(1-\frac{1}{d})U||_F \leq \frac{101}{100}\cdot \frac{17}{16}||(1-\frac{1}{d^*})\Uo||_F.$$

\begin{align*}
    \frac{16}{17}\|\frac{1}{d^*} \gradf(\Xo)\Uo\|_F &\leq \|\frac{1}{d} \gradf(\Xo)\Uo\|_F\\
    &\leq \frac{1}{d} \left(\|(\gradf(\Xo) -\gradf(X))\Uo\|_F +\|\gradf(X)\Uo\|_F \right)\\
    & \leq \frac{1}{d} \left(M\|X-\Xo\|_F \|\Uo\|_F +\|\gradf(X)(\Uo-\U)\|_F +\|\gradf(X)\U\|_F \right)\\
    &\leq \frac{1}{d} \left(\frac{M||X||}{100} \|\Uo\|_F + \|\gradf(X)\|_2\frac{1}{100} \|\U\|_F +\|\gradf(X)\U\|_F \right)\\
    &\leq \frac{1}{d} \left(\frac{1}{1600 \eta}\frac{101}{100}\|\U\|_F +\|\gradf(X)\U\|_F \right).
\end{align*}

Hence we get,
\begin{align*}
    ||(1-\frac{1}{d})U||_F &\leq \frac{101}{100}\cdot \frac{17^2}{16^2}\frac{1}{d} \left(\frac{1}{1600 }\frac{101}{100}\|\U\|_F +\eta \|\gradf(X)\U\|_F \right)
\end{align*}
The above equation implies $||(1-\frac{1}{d})U||_F \leq \frac{1.15}{d} \eta \|\gradf(X)\U\|_F $.
\end{proof}

\begin{lemma}\label{lem:supp2}
$$\ip{\gradf(X)}{X} \geq \frac{0.85}{\eta} (1-\frac{1}{d})||U||_F^2.$$ 
\end{lemma}
\begin{proof}
By first order optimality conditions we know for any feasible $X, \ip{X-\Xo}{\gradf(\Xo)} \geq 0$. Hence $$\ip{X}{\gradf(\Xo)} \geq \ip{\Xo}{\gradf(\Xo)}.$$ Further from optimality of $\Uo$ we know that $\Uo = \frac{1}{d^*}(\Uo-\eta \gradf(\Xo)\Uo).$ Hence $\ip{(1-\frac{1}{d^*})\Uo}{\Uo} =\ip{\frac{1}{d^*} \eta \gradf(\Xo)\Uo}{\Uo}$, which implies $$\ip{\Xo}{\gradf(\Xo)} =\frac{d^*}{\eta}(1-\frac{1}{d^*})||\Uo\|_F^2.$$

Finally \begin{align*}
    \ip{\gradf(X)}{X}- \ip{\gradf(\Xo)}{\X} &\geq -||\gradf(X) -\gradf(\Xo)||_F||\X||_F \\
    &\geq -M||X-\Xo||_F ||X||_F\\
    &\geq -M 2||U||_F^3 \dist(U, \Uo)\\
    &\geq -(1-\frac{1}{d})M ||U||_F^4
   % & \geq \frac{-m}{100}||X||_F^2.
\end{align*}
Last inequality follows from Lemma~\ref{lem:proj1} and using $||U -\Up||_F \leq ||U -\Uo||_F$.

Hence $\ip{\gradf(X)}{X} \geq \frac{1}{\eta} \frac{100^2 *16}{101^2 *17} (1-\frac{1}{d})||U||_F^2 -(1-\frac{1}{d})M ||U||_F^4 \geq \frac{0.85}{\eta} (1-\frac{1}{d})||U||_F^2$.
\end{proof}
\end{document}



==> proof.tex <==
%\newcommand{\algo}{\textsc{Fgd}\xspace}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\Var}{\operatorname{Var}}
%\newcommand{\eqdef}{\stackrel{\textrm{def}}{=}}
%\DeclareMathOperator{\trace}{Tr}
%\DeclareMathOperator*{\argmin}{argmin}
%\DeclareMathOperator*{\argmax}{argmax}
%\newcommand{\expec}[1]{\mathbb{E}\left[#1\right]}
%\newcommand{\prob}[1]{\mathbb{P}\left[#1\right]}
%\newcommand{\ip}[2]{\left\langle #1, #2 \right\rangle}
%\newcommand{\abs}[1]{\left \vert #1\right \vert}
%\newcommand{\norm}[1]{\left \Vert #1\right \Vert}
%\newcommand{\dist}{{\rm{\textsc{Dist}}}}
%\newcommand{\cmark}{\ding{51}}%
%
%\newcommand{\plus}[1]{{#1}^{\scalebox{0.7}{+}}}
%\newcommand{\mat}[1]{\mathbf{#1}}
%
%%% paper specific commands %%
%\newcommand{\X}{X}
%\newcommand{\Xp}{\plus{X}}
%\newcommand{\Xo}{X^{\star}}
%\newcommand{\M}{M}
%\newcommand{\U}{U}
%\newcommand{\W}{W}
%\newcommand{\B}{\mathcal{B}}
%\newcommand{\f}{f}
%\newcommand{\g}{g}
%\newcommand{\gradf}{\nabla \f}
%\newcommand{\hessf}{\nabla^2 \f}
%\newcommand{\gradg}{\nabla \g}
%\newcommand{\hessg}{\nabla^2 \g}
%\newcommand{\Vo}{V^{\star}}
%\newcommand{\Uo}{U^{\star}}
%\newcommand{\Uz}{U^0}
%\newcommand{\gu}{\gamma_u}
%\newcommand{\gl}{\gamma_l}
%\newcommand{\uut}{\U \U^{\top}}
%\newcommand{\uouot}{\Uo (\Uo)^{\top}}
%\newcommand{\Q}{Q}
%\newcommand{\Qo}{Q^{\star}}
%\newcommand{\Qs}{\Sigma}
%\newcommand{\So}{\Sigma^{\star}}
%\newcommand{\condx}{\tau(\X)}
%\newcommand{\condxo}{\tau(\Xo_r)}
%\newcommand{\rscm}{m}
%\newcommand{\rscM}{\widehat{M}}
%\newcommand{\Uor}{U^\star R}
%\newcommand{\Uorr}{U_r^\star R_U^\star}
%\newcommand{\Xor}{X^{\star}_r}
%\newcommand{\weta}{\widehat{\eta}}
%
%\def\Up{\plus{U}}
%\def\vp{V^+}
%\def\so{\sigma^*}
%\def\uo{u^*}
%\def\up{u^+}
%\def\uh{\hat{u}}
%\def\U{U}
%\def\V{V}
%\def\Q{Q}
%\def\Y{Y}
%\def\S{\mathbb{S}}
%\def\obs{\mathbf{y}}
%\def\linmap{\mathcal{A}}
%\def\w{\mathbf{w}}
%\newcommand{\cdiff}{\delta}
%\newcommand{\cdiffp}{\plus{\cdiff}}
%
%\newcommand{\Uhp}{\plus{\hat{\U}}}
%\newcommand{\Xhp}{\plus{\hat{\X}}}
%\newcommand{\tU}{\tilde{U}}
%\newcommand{\tX}{\tilde{X}}
%\newcommand{\tDelta}{\tilde{\Delta}}
%\newcommand{\PU}{\Pi_{C_U}}
%\newcommand{\PX}{\Pi_{C_X}}
%\newcommand{\gU}{g(U)}
%\newcommand{\gX}{g(X)}
%\newcommand{\tasosmargin}[1]{\marginpar{\tiny\textcolor{red}{Tasos: #1}}}

\section{Appendix C}
Here, we present the full proof of Theorem \ref{thm:projFGD_guarantees}. 
For clarity, we re-state the problem settings: We consider problem cases such as
\begin{equation*}{\label{eq:appe_00}}
\begin{aligned}
	& \underset{\X \in \R^{n \times n}}{\text{minimize}}
	& & f(\X) \\
	& \text{subject to}
	& & \X \succeq 0, ~\text{rank}(\X) \leq r^\star, ~\X \in \C',
\end{aligned}
\end{equation*} where, by definition, the optimum $\X^\star$ satisfies $\text{rank}(\X^\star) = r^\star$. For our analysis, we just use $r^\star \equiv r$. To solve \eqref{eq:appe_00}, we optimize over the re-parameterized problem:
\begin{equation*}{\label{eq:appe_01}}
\begin{aligned}
	& \underset{\U \in \R^{n \times r}}{\text{minimize}}
	& & f(\U\U^\top) \\
	& \text{subject to}
	& & \U \in \C.
\end{aligned}
\end{equation*} 
We assume $\C'$ is a convex set over $\X$ and there exists a corresponding one-to-one convex mapping onto $\C$, such that the two constraints are equivalent. As an example, consider the case where, for any $\X = \U\U^\top$, $\trace(\X) \leq 1 \Leftrightarrow \|\U\|_F^2 \leq 1$. This also implies that, if $\U \in \C$, then $\X = \U\U^\top \in \C'$. 

For our analysis, we will use the following step sizes: 
\begin{align*}
\hat{\eta} = \tfrac{1}{16(L\|\X\|_2 + \|\gradf(\X)\|_2)}, ~~\eta^\star = \tfrac{1}{16(L\|\X^\star\|_2 + \|\gradf(\X^\star)\|_2)}.
\end{align*} By Lemma A.5 in \cite{bhojanapalli2015dropping}, we know that $\hat{\eta} \geq \tfrac{5}{6} \eta$ and $\tfrac{10}{11}\eta^\star \leq \eta \leq \tfrac{11}{10} \eta^\star$. In our proof, we will work with step size $\hat{\eta}$. As noted above, this is equivalent upto constants to the original step size $\eta$ in the algorithm. 

Moreover, for ease of exposition, we re-define the sequence of updates as:
$U \equiv \U_t $, 
$\Uhp \equiv \widetilde{\U}_{t+1} = U - \hat{\eta} \gradf(X)U$ and $\Up \equiv \U_{t+1} = \Pi_{\C}(\Uhp)$. Observe that for the constraint cases we consider in this paper, $\Up = \Pi_{\C}(\Uhp) = S \cdot \Uhp$, where $S$ is a diagonal matrix with appropriate weights $\tfrac{1}{s}$ on the diagonal and $s \geq 1$. Given $\Up$, we define $\Xp = \Up\left(\Up\right)^\top$. %Define $\gU = \frac{1}{\eta}(U -\Up)$ and $\gX = \frac{1}{\eta}\left(Q_U Q_U^\top -\PU(U-\eta\gradf(X)U)U^\dagger \right)$. Then, $\gU =\gX*U$.

%Finally, our theoretical guarantees apply for the more general case where $\text{rank}(\Xo) > r$. In that case, $\Xo_r$ denotes the best rank-$r$ approximation of $\Xo$ and $\Xo_r = \U_r^\star \U_r^{\star\top}$. Thus, our theorem also proves Corollary \ref{cor:main_proof}.

\subsection{Assumptions}
%The main assumption required by \palgo for convergence are similar to that of \cite{bhojanapalli2015dropping} and can be summarized as follows: \vspace{0.3cm}

%\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \algo \textsc{Assumptions}
%\begin{itemize}[leftmargin=0.8cm] 
	%\item 
	{\it Initialization:} We assume that \palgo is initialized with a ``good'' starting point $X^0=U^0(U^0)^\top$, such that:
	\begin{itemize}
	\item [$(A1)$]  \quad \quad \quad \quad \quad  \quad \quad \quad \quad \quad$ \dist(\U^0, \Uo_r) \leq \rho' \sigma_{r}(\Uo_r)$ ~~\text{for } $\rho' := c \cdot \tfrac{\mu}{L} \cdot \tfrac{\sigma_r(\Xo)}{\sigma_1(\Xo)}  $, where $c \leq \tfrac{1}{100}$.
	\end{itemize}
	This assumption leads to a local convergence result, if no appropriate initialization is provided. Some initialization procedures that give guarantees of this type are given in \cite{bhojanapalli2015dropping}.
	
%	\item {\it Approximate rank-$r$ optimum:} Let $\Xo$ be the optimum of \eqref{eq:app_00}. In the case where we set $r < \text{rank}(\Xo) $ for computational or statistical reasons, we require:
%		\begin{itemize}
%	\item [$(A2)$]  \quad \quad \quad \quad \quad  \quad \quad \quad \quad \quad$ \|\Xo -\Xo_r\|_F \leq  c' \cdot \left(\tfrac{\mu}{L}\right)^{1.5} \cdot \tfrac{\sigma_r(\Xo)}{\sigma_1(\Xo)} \sigma_{r}(\Xo)$, 
%	\end{itemize}
%	This assumption intuitively constrains the rank constrained optimum to be closer to $\Xo_r$.
%\end{itemize}

\subsection{Supporting lemmas} 
First, we provide a series of lemmata required for the proof Theorem \ref{thm:projFGD_guarantees}. Instead of plain strong convexity, in our analysis we use \emph{restricted strong convexity}:
\begin{definition}{\label{app:def_00}}
Let $f: \R^{n \times n} \rightarrow \R$ be convex and differentiable. Then, $f$ is $(\mu, r)$-restricted strongly convex if: 
\begin{equation}\label{eq:app_sc}
f(\Y) \geq f(\X) + \ip{\gradf\left(\X\right)}{\Y - \X} + \tfrac{\mu}{2} \norm{Y - \X}_F^2,
\end{equation} $\forall \X, \Y \in  \R^{n \times n}$, rank-$r$ matrices.
\end{definition}

The statements below apply equally for plain $\mu$-strong convexity, as defined in Definition \ref{prelim:def_00}.

\begin{lemma}\label{app_lem:gradX,X-X_r_ bound_sc}
Let $f$ be a $L$-smooth and $(\mu, r)$-restricted strongly convex function with optimum point $\Xo$. Then,
\begin{align*}   
\ip{\gradf(\X)}{\X-\Xo}  \geq &\tfrac{17}{16\eta} \|U -\Up\|_F^2 + \tfrac{3\cdot\eta}{5 s^2} \cdot \|\gradf(X) U\|_F^2  + \tfrac{\mu}{2}\norm{\X - \Xo}_F^2 +\tfrac{1}{20 \eta}\left(1-\tfrac{1}{s}\right)\|U\|_F^2.
\end{align*}
\end{lemma}

\begin{proof}
Following similar motions with \cite{bhojanapalli2015dropping}, by smoothness of $\f$, we get:
\begin{align}
\f(\X) &\geq \f(\Xp) -\ip{\gradf(\X)}{\Xp -\X} - \tfrac{L}{2} \norm{\Xp -\X}_F^2 \nonumber \\ 
&\stackrel{(i)}{\geq} \f(\Xo) -\ip{\gradf(\X)}{\Xp -\X} - \tfrac{L}{2} \norm{\Xp -\X}_F^2 , \label{eq:gradX,X-X_r_00}
 \end{align}
where $(i)$ follows from optimality of $\Xo$ and since $\Xp$ is a feasible point $(\Xp \succeq 0, ~\Pi_{\C'}(\Xp) = \Xp)$ for problem~\eqref{eq:appe_00}. Here, we remind that $\Xp = \Up\left(\Up\right)^\top$ and we use the fact that, since $\Up \in \C$ then $\Xp \in \C'$. 
%Further, applying again smoothness of $f$, we have:
%\begin{align}
%asd
%\end{align}

Moreover, by the $(\mu, r)$-restricted strong convexity of $\f$, we get, 
\begin{align} 
\f(\Xo) \geq \f(\X) +\ip{\gradf(\X)}{\Xo-\X} +\tfrac{\mu}{2}\norm{\Xo -\X}_F^2 .\label{eq:gradX,X-X_r_02}
\end{align}
Combining equations~\eqref{eq:gradX,X-X_r_00}, and~\eqref{eq:gradX,X-X_r_02}, we obtain: 
\begin{align} 
\ip{\gradf(\X)}{\X-\Xo} \geq  \ip{\gradf(\X)}{\X -\Xp} -\tfrac{L}{2} \norm{\Xp -\X}_F^2+\tfrac{\mu}{2}\norm{\Xo -\X}_F^2  \label{eq:gradX,X-X_r_03} 
\end{align}
It is easy to verify that $\Xp =  \frac{1}{s^2}\left(\X - \eta \gradf(\X) \X \Lambda - \eta \Lambda^\top \X \gradf(\X)\right)$, where $\Lambda = I - \tfrac{\eta}{2} Q_U Q_U^\top \gradf(X) \in \R^{n \times n}$ and $Q_\U Q_\U^\top$ denoting the projection onto the column space of $\U$.
%In the proof that follows, we use as step size $\widehat{\eta} = \tfrac{1}{16 (M\|\X\|_2 + \|\gradf(\X)Q_U Q_U^\top\|_2)}$. 
%By Lemma \ref{lem:stepsize}, we can verify that $\widehat{\eta} \geq \eta$ and, thus, any theoretical result using $\widehat{\eta}$ as step size automatically applies for the proposed step size $\eta$. 
Notice that, for step size ${\eta}$, we have 
\begin{align*}
\Lambda \succ 0, \quad  \|\Lambda\|_2 \leq  1+ \sfrac{1}{32} \quad \text{and} \quad \sigma_{n}(\Lambda) \geq  1- \sfrac{1}{32}.
\end{align*} 

%Now recall that \begin{align*}\Xp &= X - \weta \gradf(X)X -  \weta X \gradf(X)+  \weta^2 \gradf(X)X \gradf(X) \\
%&= X - \weta \left( \gradf(X)X\Lambda  + \Lambda^\top X \gradf(X) \right), \end{align*} where $\Lambda =I -\frac{\weta}{2} Q_{U} Q_{U}^\top \gradf(X)$. Notice that for step size $\weta$ considered $\Lambda \succ 0$,  $\|\Lambda\|_2 \leq  1+ \frac{1}{32}$ and $\sigma_{n}(\Lambda) \geq  1- \frac{1}{32}$.

Substituting the above in~\eqref{eq:gradX,X-X_r_03}, we obtain:
\begin{align}\label{eq:appe_000}
 \ip{\gradf(\X)}{\X-\Xo} &- \tfrac{\mu}{2}\norm{\Xo -\X}_F^2 + \tfrac{L}{2} \norm{X -\Xp}_F^2 \nonumber \\
 								 &\stackrel{(i)}{\geq} \ip{\gradf(X)}{\left(1-\tfrac{1}{s^2}\right)X} + 
 								 \tfrac{2\eta}{s^2} \cdot \ip{\gradf(\X)}{\gradf(X)X \Lambda} \nonumber \\
 								 &\stackrel{(ii)}{\geq} \ip{\gradf(X)U}{\left(1-\tfrac{1}{s^2}\right)U} + \tfrac{2\eta}{s^2} \cdot \trace( \gradf(X) \gradf(X)X) \cdot \sigma_{n}(\Lambda) \nonumber \\
 								 &\geq \left(1-\tfrac{1}{s^2}\right) \cdot \ip{\gradf(X)}{X} + \tfrac{31\cdot\eta}{16 s^2} \|\gradf(X) U\|_F^2,
 \end{align} 
where: $(i)$ follows from symmetry of $\gradf(X)$ and $\X$ and, $(ii)$ follows from the sequence equalities an inequalites: $\trace(\gradf(X)\gradf(X)X\Lambda) =\trace(\gradf(X)\gradf(X)UU^\top) -\frac{\eta}{2}\trace(\gradf(X)\gradf(X)UU^\top \gradf(X)) \geq (1 -\frac{\eta}{2} \|Q_U Q_U^\top\gradf(X)\|_2) \|\gradf(\X) U\|_F^2  \geq  (1- \sfrac{1}{32}) \|\gradf(\X) U\|_F^2$.  %$(iii)$ follows by $\weta \leq \tfrac{1}{16M \|\X\|_2}$. Thus, we achieve the desiderata:
 
The term $\tfrac{L}{2} \norm{X -\Xp}_F^2$ can be bounded as follows:
\begin{align*}
\tfrac{L}{2} \norm{X -\Xp}_F^2 
\end{align*}
Using this bound in \eqref{eq:appe_000} and adding $-\frac{17}{16\eta} \|U -\Up\|_F^2$ in both sides we get:
 \begin{align*}
     \ip{\gradf(\X)}{\X-\Xo} &- \tfrac{\mu}{2}\norm{\Xo - \X}_F^2 -\tfrac{17}{16\eta} \|U -\Up\|_F^2\\
     &\geq  \left(1-\frac{1}{s^2}\right)\ip{\gradf(X)}{X} + \tfrac{31\cdot\eta}{16 d^2} \|\gradf(X) U\|_F^2 - \left(1+ \tfrac{1}{32} \right) \cdot \frac{17}{16\eta} \cdot \|U -\Up\|_F^2\\
     &\geq  (1-\frac{1}{d^2})\ip{\gradf(X)}{X} + \tfrac{31\cdot\eta}{16 d^2} \|\gradf(X) U\|_F^2 \\
     &\quad -\frac{33}{32}\frac{17}{16 \eta}\left[(1-\frac{1}{d})^2\|U\|_F^2 + \frac{\eta^2}{d^2}\|\gradf(X)U\|_F^2 + 2\eta \frac{1}{d} (1-\frac{1}{d}) \ip{\gradf(X)}{X} \right]\\
     &\geq (1-\frac{1}{d})(1+\frac{1}{34d})\ip{\gradf(X)}{X} + \tfrac{0.96\cdot\eta}{ d^2} \|\gradf(X) U\|_F^2 -\frac{33*17}{32*16 \eta}(1-\frac{1}{d})^2\|U\|_F^2\\
     &\stackrel{(i)}{\geq} (1+\frac{1}{34d}) \frac{0.85}{\eta}(1-\frac{1}{d})^2\|U\|_F^2 + \tfrac{0.96\cdot\eta}{ d^2} \|\gradf(X) U\|_F^2 -\frac{33*17}{32*16 \eta}(1-\frac{1}{d})^2\|U\|_F^2\\
     &\stackrel{(ii)}{\geq} \tfrac{0.96\cdot\eta}{ d^2} \|\gradf(X) U\|_F^2 - \frac{0.22}{\eta}(1-\frac{1}{d})^2\|U\|_F^2\\
     &\geq \frac{3\cdot\eta}{5 d^2} \|\gradf(X) U\|_F^2 +\frac{1}{20 \eta}(1-\frac{1}{d})\|U\|_F^2.
 \end{align*}
 $(i)$ follows from applying Lemma~\ref{lem:supp2}. $(ii)$ follows from $d \leq \frac{17}{16}$. Last inequality follows from Lemma~\ref{lem:proj1} and  $(1-\frac{1}{d^2}) \leq (1-\frac{1}{d})$.
\end{proof}


\begin{lemma}[Descent lemma]\label{lem:gradU,U-U_r_ bound}
Let $f$ be a $L$-smooth and $(\mu, r)$-strongly convex function. Then, under assumptions $(A1)$ and $(A2)$, the following inequality holds true:
\begin{align*}
\ip{\gradf(X)U}{\U -\Uorr} \geq  &\tfrac{17}{16\eta} \|U -\Up\|_F^2 + \tfrac{47 \cdot \eta}{160}  \|\gradf(X) U\|_F^2 + \tfrac{3\mu}{20} \cdot  \sigma_{r}(\Xo) \cdot \dist(\U, \Uo_r)^2 \\&\quad \quad +\tfrac{1}{20 \eta}\left(1-\tfrac{1}{s}\right)\|U\|_F^2 -\tfrac{L}{4}\norm{\Xo -\Xor}_F^2 .
\end{align*}
\end{lemma}

\begin{proof}
Recall $\Uhp =U -\eta\gradf(X)U$ and define $\Delta := \U - \Uo_r \R_{\U}^\star$. First we rewrite the inner product as shown below.
\begin{align}
\ip{\gradf(X)U}{\U -\Uorr}&= \ip{\gradf(X) }{\X -\Uorr \U^\top} \nonumber \\
&=\frac{1}{2}\ip{\gradf(X) }{\X -\Xo_r}  + \ip{\gradf(X) }{\frac{1}{2}(\X + \Xo_r) -\Uorr \U^\top} \nonumber \\
&=\frac{1}{2}\ip{\gradf(X) }{\X -\Xo_r}  + \frac{1}{2} \ip{\gradf(X) }{\Delta \Delta^\top}, \label{proofsr1:eq_09}
\end{align} which follows by adding and subtracting $\tfrac{1}{2}\Xo_r$. 
We know by Lemma C.1 in \cite{bhojanapalli2015dropping} that $\ip{\gradf(X) }{\Delta \Delta^\top} \leq \frac{\mu \cdot \sigma_r(\Xo_r)}{40 \cdot L \cdot \sigma_1(\Xo_r)} \cdot \|\gradf(X)U\|_F \cdot \dist(U, \Uo_r)$. Combining the above with Lemmas ??\ref{lem:DD_bound} and \ref{lem:gradX,X-X_r_ bound}, we have:

\begin{align*}
& \ip{\gradf(X) \U}{\U -\Uorr}\\ &\geq \frac{17}{16\eta} \|U -\Up\|_F^2 + \tfrac{3\cdot\eta}{5 d^2} \|\gradf(X) U\|_F^2 + \tfrac{m}{4}\norm{\X -\Xor}_F^2 +\frac{1}{20 \eta}(1-\frac{1}{d})\|U\|_F^2 - \tfrac{M}{4}\norm{\Xo -\Xor}_F^2 \\
&\quad \quad \quad \quad \quad \quad \quad \quad- \tfrac{1}{2}\tfrac{1}{80 \kappa \tau(\Xo_r)}\left(   \eta\|\gradf(X)U\|_F^2 + \frac{1}{\eta}\|\Delta\|_F^2 \right) \nonumber \\
&= \frac{17}{16\eta} \|U -\Up\|_F^2 + \left(\tfrac{3}{5*2}- \tfrac{1}{160}\right) \cdot \eta  \|\gradf(X) U\|_F^2 + \tfrac{m}{4}\left(\norm{\X -\Xor}_F^2 -  \tfrac{1\sigma_{r}(\Xo) }{40} \cdot \| \Delta\|_F^2 \right) \nonumber \\ 
&\quad \quad \quad \quad \quad \quad \quad \quad +\frac{1}{20 \eta}(1-\frac{1}{d})\|U\|_F^2 - \tfrac{M}{4}\norm{\Xo -\Xor}_F^2 \nonumber \\
&\stackrel{(i)}{\geq} \frac{17}{16\eta} \|U -\Up\|_F^2 + \frac{47 \cdot \eta}{160}  \|\gradf(X) U\|_F^2 + \tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 +\frac{1}{20\eta}(1-\frac{1}{d})\|U\|_F^2 -\tfrac{M}{4}\norm{\Xo -\Xor}_F^2 \nonumber 
%&\stackrel{(ii)}{\geq }\frac{1}{ \eta} \|U- \Up\|_F^2 + \tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 - \tfrac{M}{4}\norm{\Xo -\Xor}_F^2
\end{align*}
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}\label{lem:proj}
$$\|(1-\frac{1}{d})U\|_F \leq (1+\frac{1}{d})\eta \|\gradf(X) U\|_F.$$
\end{lemma}
\begin{proof}
Recall that $\Up=\frac{1}{d}(U -\eta \gradf(X)U)$ is a projection of $\Uhp =U -\eta\gradf(X)U$. Hence $$\|U-\Up\|_F \leq \|U - \Uhp\|_F.$$ This implies,
\begin{align*}
    \weta \|\gradf(X)U\|_F &\geq \|U -\Up\|_F \\
    &\geq \|(1-\frac{1}{d})U\|_F - \frac{1}{d}\eta \|\gradf(X)U\|_F.
\end{align*}
Hence $\|(1-\frac{1}{d})U\|_F \leq (1+\frac{1}{d})\eta \|\gradf(X)U\|_F.$
\end{proof}


\begin{lemma}\label{lem:proj1}
$$\|(1-\frac{1}{d})U\|_F \leq \frac{1.15}{d} \eta \|\gradf(X) U\|_F,$$ %when $\|(1-\frac{1}{d})U\|_F \geq \frac{\kappa \tau(\Xo_r)}{50} \dist(U, \Uo)$.
\end{lemma}
\begin{proof}
From optimality of $\Uo$ we know that $\Uo = \frac{1}{d^*}(\Uo-\eta \gradf(\Xo)\Uo).$ Hence $\|(1-\frac{1}{d^*})\Uo\|_F = \|\frac{1}{d^*} \eta \gradf(\Xo)\Uo\|_F.$ Notice that $d^* \geq 1 \geq \frac{16}{17}d$, since $d \leq \frac{17}{16}$. Also $\|\U\|_F \leq \frac{101}{100}\|\Uo\|_F$ from lemma {\color{red} ref}. Hence we get,
$$\|(1-\frac{1}{d})U\|_F \leq \frac{101}{100}\cdot \frac{17}{16}\|(1-\frac{1}{d^*})\Uo\|_F.$$

\begin{align*}
    \frac{16}{17}\|\frac{1}{d^*} \gradf(\Xo)\Uo\|_F &\leq \|\frac{1}{d} \gradf(\Xo)\Uo\|_F\\
    &\leq \frac{1}{d} \left(\|(\gradf(\Xo) -\gradf(X))\Uo\|_F +\|\gradf(X)\Uo\|_F \right)\\
    & \leq \frac{1}{d} \left(M\|X-\Xo\|_F \|\Uo\|_F +\|\gradf(X)(\Uo-\U)\|_F +\|\gradf(X)\U\|_F \right)\\
    &\leq \frac{1}{d} \left(\frac{M\|X\|}{100} \|\Uo\|_F + \|\gradf(X)\|_2\frac{1}{100} \|\U\|_F +\|\gradf(X)\U\|_F \right)\\
    &\leq \frac{1}{d} \left(\frac{1}{1600 \eta}\frac{101}{100}\|\U\|_F +\|\gradf(X)\U\|_F \right).
\end{align*}

Hence we get,
\begin{align*}
    \|(1-\frac{1}{d})U\|_F &\leq \frac{101}{100}\cdot \frac{17^2}{16^2}\frac{1}{d} \left(\frac{1}{1600 }\frac{101}{100}\|\U\|_F +\eta \|\gradf(X)\U\|_F \right)
\end{align*}
The above equation implies $\|(1-\frac{1}{d})U\|_F \leq \frac{1.15}{d} \eta \|\gradf(X)\U\|_F $.
\end{proof}

\begin{lemma}\label{lem:supp2}
$$\ip{\gradf(X)}{X} \geq \frac{0.85}{\eta} (1-\frac{1}{d})\|U\|_F^2.$$ 
\end{lemma}
\begin{proof}
By first order optimality conditions we know for any feasible $X, \ip{X-\Xo}{\gradf(\Xo)} \geq 0$. Hence $$\ip{X}{\gradf(\Xo)} \geq \ip{\Xo}{\gradf(\Xo)}.$$ Further from optimality of $\Uo$ we know that $\Uo = \frac{1}{d^*}(\Uo-\eta \gradf(\Xo)\Uo).$ Hence $\ip{(1-\frac{1}{d^*})\Uo}{\Uo} =\ip{\frac{1}{d^*} \eta \gradf(\Xo)\Uo}{\Uo}$, which implies $$\ip{\Xo}{\gradf(\Xo)} =\frac{d^*}{\eta}(1-\frac{1}{d^*})\|\Uo\|_F^2.$$

Finally \begin{align*}
    \ip{\gradf(X)}{X}- \ip{\gradf(\Xo)}{\X} &\geq -\|\gradf(X) -\gradf(\Xo)\|_F\|\X\|_F \\
    &\geq -M\|X-\Xo\|_F \|X\|_F\\
    &\geq -M 2\|U\|_F^3 \dist(U, \Uo)\\
    &\geq -(1-\frac{1}{d})M \|U\|_F^4
   % & \geq \frac{-m}{100}\|X\|_F^2.
\end{align*}
Last inequality follows from Lemma~\ref{lem:proj1} and using $\|U -\Up\|_F \leq \|U -\Uo\|_F$.

Hence $\ip{\gradf(X)}{X} \geq \frac{1}{\eta} \frac{100^2 *16}{101^2 *17} (1-\frac{1}{d})\|U\|_F^2 -(1-\frac{1}{d})M \|U\|_F^4 \geq \frac{0.85}{\eta} (1-\frac{1}{d})\|U\|_F^2$.
\end{proof}

\begin{theorem}
$$\dist(\Up, \Uor)^2 \leq (1 -\frac{3m \sigma_r(\Xo)\eta}{10}) \| \Delta\|_F^2+ \frac{17M \eta}{32} \norm{\Xo -\Xor}_F^2.$$
\end{theorem}

\begin{proof}


\begin{align*}
    \dist(\Up,\Uor)^2 &\leq \|\Up -\Uor\|_F^2 \\
    &=\|\Up-U+U-\Uor\|_F^2\\
    &=\|\Up -U\|_F^2 +\|U-\Uor\|_F^2-2\ip{U-\Up}{U-\Uor}.
    %&=\|U-\Uor\|_F^2-\|\Up -U\|_F^2 -2\ip{U-\Up}{\Up-\Uor}\\
   % &\leq \|U-\Uor\|_F^2-\|\Up -U\|_F^2 -2\ip{U-\Uhp}{\Up-\Uor}.
\end{align*}
%For the last step, recall $\Up$ is projection of $\Uhp$. Hence, $\ip{\Uhp-\Up}{\Up -\Uor} \geq 0$. This implies, $\ip{U-\Up}{\Up -\Uor} \geq \ip{U - \Uhp}{\Up -\Uor}$.

Now we will bound the inner product in the above.
\begin{align*}
    \ip{U-\Up}{\U-\Uor}&=\ip{U-D(U-\eta\gradf(X)U)}{\U-\Uor}\\
    &=\ip{U-DU}{\U -\Uor}+\eta\ip{D\gradf(X)U}{\U-\Uor}.
\end{align*}
Now using Lemma~\ref{lem:gradU,U-U_r_ bound} we get,
\begin{align*}
      \dist(\Up,\Uor)^2 &\leq \|\Up -U\|_F^2 +\|U-\Uor\|_F^2-2\ip{U-DU}{\U -\Uor} \\ &\quad\quad -\frac{2\eta}{d} \left(\frac{17}{16\eta} \|U- \Up\|_F^2  +\tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2 +\frac{1}{20\eta}(1-\frac{1}{d})\|U\|_F^2- \tfrac{M}{4}\norm{\Xo -\Xor}_F^2\right) \\
      &\leq \|\Up -U\|_F^2 +\|U-\Uor\|_F^2 + \frac{2}{100}(1-\frac{1}{d}) \|U\|_F^2  \\ &\quad \quad -\frac{2*17\eta}{16} \left(\frac{17}{16\eta} \|U- \Up\|_F^2 +\frac{1}{20 \eta}(1-\frac{1}{d})\|U\|_F^2 +\tfrac{3m}{20} \cdot  \sigma_{r}(\Xo)  \| \Delta\|_F^2- \tfrac{M}{4}\norm{\Xo -\Xor}_F^2\right) \\
      &\leq (1 -\frac{3m \sigma_r(\Xo)\eta}{10}) \| \Delta\|_F^2+ \frac{17 M \eta}{32} \norm{\Xo -\Xor}_F^2  +\left(\tfrac{2}{100} -\tfrac{17}{160} \right)(1-\tfrac{1}{d}) \|U\|_F^2  \\
      &\leq \leq (1 -\frac{3m \sigma_r(\Xo)\eta}{10}) \| \Delta\|_F^2+ \frac{17 M \eta}{32} \norm{\Xo -\Xor}_F^2
\end{align*}
\end{proof}


==> transform.tex <==

\subsection{Transforming \eqref{eq: orig QT} into a factored formulation.} 
Before we continue our discussions, let us first show how \eqref{eq: orig QT} can be transformed in a form similar to \eqref{intro:eq_00}. For this purpose, we state the following Lemma.

\begin{lemma}{\label{lem:transform_00}}
Consider the following problem:
\begin{equation}{\label{transform:eq_00}}
\begin{aligned}
	& \underset{\X \in \R^{n \times n}}{\text{{\rm minimize}}}
	& & f(\X) \\
	& \text{{\rm subject to}}
	& & \text{{\rm rank}}(\X) = r \\
	& & & \X \succeq 0, \trace(\X) \leq 1,
\end{aligned}
\end{equation} where $f$ is a strongly convex and gradient Lipschitz continuous function.
Then, by changing the variable according to the rule $\X = \U\U^\top$, where $\U \in \R^{n \times r}$, the following problem re-formulation:
\begin{equation}{\label{transform:eq_01}}
\begin{aligned}
	& \underset{\U \in \R^{n \times r}}{\text{{\rm minimize}}}
	& & f(\U\U^\top) \\
	& \text{{\rm subject to}}
	& &\|\U\|_F^2 \leq 1.
\end{aligned}
\end{equation} is ``equivalent".
\end{lemma} 
By ``equivalent'' we mean that this change of variables does not introduce
any \emph{extraneous} local minima. 

\begin{proof}
First of all, it is obvious that, due to the matrix factorization $\X = \U\U^\top$, $\trace(\X) \leq 1 \Rightarrow \trace(\U\U^\top) \leq 1 \Rightarrow \|\U\|_F^2 \leq 1$. Then, all three constraints in \eqref{transform:eq_00} can be captured by the change of variables and the constraint $ \|\U\|_F^2 \leq 1$ in \eqref{transform:eq_01}.

Regarding the ``equivalency", the proof is heavily based on Section 2 of \cite{burer2005local}; here we sketch the proof for the general case of any 
$f$ convex function. Next, we state two important lemmas that we require for the proof of Lemma \ref{lem:transform_00}.

\begin{lemma}{\label{lem:transform_01}}
Let $\U, \V \in \R^{n \times r}$ such that $\U\U^\top = \V\V^\top$. Then, $\U = \V R$ for some orthogonal
rotation matrix $R \in \R^{n \times r}$.
\end{lemma}

\begin{lemma}{\label{lem:transform_02}}
Let $\U \in \R^{n \times r}$ be a local minimum of \eqref{transform:eq_01}. Then, $\U R$ is also a local minimum, 
for all orthogonal matrices $R \in \R^{n \times r}$
\end{lemma}

Let us denote $\widehat{\X}$ a feasible point of \eqref{transform:eq_00}; moreover, let $\X = \widehat{\U} \widehat{\U}^\top$ 
for $\widehat{\U} \in \R^{n \times r}$, which further implies that $\widehat{\U}$ is feasible for \eqref{transform:eq_01}. 
We next prove that if $\widehat{\X}$ is a local minimum of \eqref{transform:eq_00}, so is $\widehat{\U}$ for \eqref{transform:eq_01} 
(if and only if statement).

By continuity of the map $\U \mapsto \U\U^\top $, it is easy to observe that if $\widehat{\X}$ is a local 
minimum of \eqref{transform:eq_00}, then each $\U$ satisfying $\X = \U\U^\top$ is a local minimum of \eqref{transform:eq_01}. 
Then, due to Lemma \ref{lem:transform_01}, there is a rotational matrix $R$ such that $\widehat{\U} = \U R$. 

Now, assume that $\widehat{\X}$ is not a local minimum of \eqref{transform:eq_00}, and thus there is a sequence of 
feasible solutions $\left\{\X^k\right\}$ for \eqref{transform:eq_00} that converge to $\widehat{\X}$ and have smaller 
objective value (since $f$ is a convex function). \textit{I.e.}, $f(\X^k) < f(\widehat{\X})$, for all $k$. Since all 
points in $\{\X^k\}$ are feasible, there are factors $\U^k$ for each $k$ such that $\X^k = \U^k \left(\U^k\right)^\top$.
Moreover, for bounded $\{\X^k\}$, we imply that also $\{\U^k\}$ is bounded and, therefore, there is a sequence
of factors that converge to some $\U$, such that $\widehat{\X} = \U\U^\top$. By assumption, the following 
sequence of inequalities apply: $f(\U^k(\U^k)^\top) = f(\X^k) < f(\widehat{\X}) = f(\U\U^\top)$; thus, $\U$ is also
not a local minimum of \eqref{transform:eq_01}. This observation, combined with Lemmata \ref{lem:transform_00}-\ref{lem:transform_01},
points to the conclusion that $\widehat{\U}$ is not a local minimum, when $\widehat{\X}$ is not a local minimum.
\end{proof}

%The constraint set of \eqref{transform:eq_01} can be re-written as $\|\U\|_F^2 \leq 1$, \textit{i.e.}, it is a convex projection
%on the unit ball  in $\R^{n \times r}$. 


